Fast Adaptation with Meta-Reinforcement Learning for Trust Modelling in Human-Robot Interaction

In socially assistive robotics, an important research area is the development of adaptation techniques and their effect on human-robot interaction. We present a meta-learning based policy gradient method for addressing the problem of adaptation in human-robot interaction and also investigate its role as a mechanism for trust modelling. By building an escape room scenario in mixed reality with a robot, we test our hypothesis that bi-directional trust can be influenced by different adaptation algorithms. We found that our proposed model increased the perceived trustworthiness of the robot and influenced the dynamics of gaining human's trust. Additionally, participants evaluated that the robot perceived them as more trustworthy during the interactions with the meta-learning based adaptation compared to the previously studied statistical adaptation model.

==> introduction_bk.tex <==
% %%%%%% motivation for adaptation in hri %%%%%% 
% Robots are no longer viewed only as machines restricted to isolated compounds and dangerous to people. The idea of robot as a companion is gaining its momentum and popularity not only in research community, but also in public perception. But in order to navigate in complex environment and ever changing dynamics of human-robot interactions, robots need to be able to learn and adapt. For example, an assistive robot that helps elderly people is assumed to be able to understand the person's need, perform basic manipulation tasks, and also provide emotional support when needed. Furthermore, humans are intelligent agents that have their own internal state, which changes through out the interaction. Thus, the need to learn and adapt in the dynamic environment is essential to enable smooth human-robot interaction. 

{\color{red}
%%%%%% psychological background: conation, cognition, affection introduction %%%%%% 
Adaptation in dynamic environments is essential to enable smooth human-robot interaction and still remains a challenge \cite{sheridan2016human}.
There exists an extensive body of work on application-driven adaptation in human-robot interaction. 
%TODO: expand this brief overview
Recent developments have explored different aspects of human robot interaction including physical human-robot interaction ~\cite{ghadirzadeh2016sensorimotor}, automatic reasoning~\cite{clark2018deep} and affective human-robot interaction~\cite{yuan2018when}
All these methods are successful in their own field, but also view the human-robot interaction process from a narrow perspective.
In our paper, however, we want to present a more general approach to adaptation in human-robot interaction based on the tripartite classification of mental activities of human personality and intelligence into \textit{conation}, \textit{cognition}, and \textit{affection} ~\cite{hilgard1980trilogy} and using meta reinforcement learning process as trust modelling. For example, an assistive robot that helps elderly people performs an instance of \textit{conation} by identifying human's intent, a manipulation task corresponds to an instance of \textit{cognition}, while \textit{affection} is provided as emotional support. 

%%%%%% model formulation %%%%%% 
In order to implement fast adaptation for a robot in dynamic environment, we formulate the tripartite classification based approach to human-robot interaction as a deep reinforcement learning problem alongside with model-agnostic meta-learning for higher-level control over all the different mental activities. In Section \ref{sec:Method}, we provide a formal description of our model. 
% TODO: provide reasoning why. (IMPORTANT: discuss it with Alex)


%%%%%% scenario %%%%%% 
We evaluate our model on a human-robot interaction scenario where a human participant has to collaborate with a robot in order to escape a room, recreated with mixed reality. The room is separated by a virtual half-transparent wall that both robot and human are not able to trespass. The participant need a "key" to get out but all "keys" are placed in the robot's part of the room. Keys are represented as different objects. The participant has to ask the robot to bring them the correct object to open an escape door. From speech and human's 3D position in space, the robot learns intentions of the participants, new objects, and supportive behavior. Our scenario is discussed in more details in the Section [ref scenario].

% TODO: update this after our experiment
For the escape room scenario, both objective and subjective measures were considered in a between-group human study, such as model accuracy, participant's task performance and stress level. As discussed in the section [ref results], the results showed… 
% TODO: add results later

%%%%%% main contribution %%%%%% 
% TODO: add main contribution later
}

==> introduction_old.tex <==
% Human robot interaction has became an emerging field over the years and in order to achieve smooth interaction experiences, many different techniques have been employed to endure intelligence on robots. Deep reinforcement learning is one of the most successful methods in recent years. Recent developments explored different aspects of human robot interaction including physical human-robot interaction ~\cite{ghadirzadeh2016sensorimotor}, automatic reasoning~\cite{clark2018deep} and affective human-robot interaction~\cite{gao2018robot}. These methods are successful in their own field but also view the human robot interaction process from a narrow angle. 

%%%%%% motivation for adaptation in hri %%%%%% 
Robots are no longer viewed only as machines restricted to isolated compounds and dangerous to people. The idea of robot as a companion is gaining its momentum and popularity not only in research community, but also in public perception. But in order to navigate in complex environment and ever changing dynamics of human-robot interactions, robots need to be able to learn and adapt. For example, an assistive robot that helps elderly people is assumed to be able to understand the person's need, perform basic manipulation tasks, and also provide emotional support when needed. Furthermore, humans are intelligent agents that have their own internal state, which changes through out the interaction. Thus, the need to learn and adapt in the dynamic environment is essential to enable smooth human-robot interaction. 

%%%%%% psychological background: conation, cognition, affection introduction %%%%%% 
There exists an extensive body of work on application-driven adaptation in human-robot interaction. 
%TODO: expand this brief overview
Recent developments explored different aspects of human robot interaction including physical human-robot interaction ~\cite{ghadirzadeh2016sensorimotor}, automatic reasoning~\cite{clark2018deep} and affective human-robot interaction~\cite{gao2018robot}
All these methods are successful in their own field, but also view the human-robot interaction process from a narrow perspective.
In our paper, however, we want to present a more general approach to adaptation in human-robot interaction based on the tripartite classification of mental activities of human personality and intelligence into \textit{conation}, \textit{cognition}, and \textit{affection} ~\cite{hilgard1980trilogy} and using meta reinforcement leanring process as trust modelling. From the previous example with an assistive robot, an act of intent recognition corresponds to \textit{conation}, while \textit{cognition} is performed through a manipulation task, and \textit{affection} is provided as emotional support. 

%%%%%% model formulation %%%%%% 
In order to implement fast adaptation for a robot in dynamic environment, we formulate the tripartite classification based approach to human-robot interaction as a deep reinforcement learning problem alongside with model-agnostic meta-learning for higher-level control over all the different mental activities. In Section \ref{sec:Method}, we provide a formal description of our model. 
% TODO: provide reasoning why. (IMPORTANT: discuss it with Alex)


%%%%%% scenario %%%%%% 
We evaluate our model on a multimodal interaction scenario where a human participant has to collaborate with a robot in order to escape a room recreated with augmented reality. The room is separated by a virtual half-transparent wall that both robot and human are not able to trespass. The participant need a "key" to get out but all "keys" are placed in the robot's part of the room. Keys are represented as different objects. The participant has to ask the robot to bring them the correct object to open an escape door. From speech and human's 3D position in space, the robot learns intentions of the participants, new objects, and supportive behavior. Our scenario is discussed in more details in the Section [ref scenario].

% TODO: update this after our experiment
For the escape room scenario, both objective and subjective measures were considered in a between-group human study, such as model accuracy, participant's task performance and stress level. As discussed in the section [ref results], the results showed… 
% TODO: add results later

%%%%%% main contribution %%%%%% 
% TODO: add main contribution later
